Data-Driven Abductive Inference of Library Specifications

Programmers often leverage data structure libraries that provide useful and reusable abstractions. Modular verification of programs that make use of these libraries naturally rely on specifications that capture important properties about how the library expects these data structures to be accessed and manipulated. However, these specifications are often missing or incomplete, making it hard for clients to be confident they are using the library safely. When library source code is also unavailable, as is often the case, the challenge to infer meaningful specifications is further exacerbated. In this paper, we present a novel data-driven abductive inference mechanism that infers specifications for library methods sufficient to enable verification of the library's clients. Our technique combines a data-driven learning-based framework to postulate candidate specifications, along with SMT-provided counterexamples to refine these candidates, taking special care to prevent generating specifications that overfit to sampled tests. The resulting specifications form a minimal set of requirements on the behavior of library implementations that ensures safety of a particular client program. Our solution thus provides a new multi-abduction procedure for precise specification inference of data structure libraries guided by client-side verification tasks. Experimental results on a wide range of realistic OCaml data structure programs demonstrate the effectiveness of the approach.

==> discuss/1.tex <==
I understood your worry, that is, even I got a "maximal specification mapping" with respect to my definition, what appears on the left hand of $\models$(the conjunctions of specifications) is not maximal. I believe this situation will happen, although I didn't come up with an example now(should be a nonlinear case with some tricky calling arguments). However, I think we have no reason to force the conjunction of the specifications to be maximal, which is not required by the ordering definition(shown in def 3.11 in our shared overleaf project). This definition is exactly the same as MMS(def 2). Moreover, I do not believe MMS can sat this requirement. Although they truly infer a merged maximal abduction result for all specifications, however, during the "decomposition" phase, they do another literately abduction to infer $R$ in $R \land \bigwedge R_{fixed} \implies merged\_result$ from initial solution. There is no guarantee that $R_{inferred} \land \bigwedge R_{fixed}$ is equal to $ merged\_result$ or the closest one to $merged\_result$ comparing with other conjunction which has different $R_{fixed}$. This may be interfered by the order of decomposition. It is the same as my algorithm which does not guarantee the maximality of the conjunction of specifications.

==> discuss/2.tex <==
I try to solve the single weakening procedure from another direction, why not design a semi-QE algorithm just fit our situation, that is, only eliminate the universal quantified datatype variables. 

Here I have an example. Assume the predicate set is ${p: a\ list \to a \to bool}$, then VC is
\begin{align*}
    P(x, y) \land Q(y, z) \implies (\forall v, p(x, v) \implies p(z, v))
\end{align*}
We fixed $Q(y,z)$ as $\forall u, p(y, u) \implies p(z, u)$, and try to find a maximal $P(x,y)$. We can easily guess that the solution is $\forall u, p(x, u) \implies p(y, u)$. The safety proving is trivial, just send
\begin{align*}
&\neg(\\
&\quad(\forall u, p(x, u) \implies p(y, u)) \land (\forall u, p(y, u) \implies p(z, u)) \implies \\
&\quad(\forall v, p(x, v) \implies p(z, v))\\
&)
\end{align*}
to SMT solver, but how can we prove the maximality? Intuitively, the query is
\begin{align*}
&\neg(\forall x\ y,\\
&\quad((\forall z, \forall u, p(y, u) \implies p(z, u)) \implies (\forall v, p(x, v) \implies p(z, v))) \implies \\
&\quad \Delta[P](x, y)\\
&)
\end{align*}
which is
\begin{align*}
&\exists x\ y,\\
&\quad(\forall z, (\forall u, p(y, u) \implies p(z, u)) \implies (\forall v, p(x, v) \implies p(z, v))) \land \\
&\quad \neg \Delta[P](x, y)
\end{align*}
or
\begin{align*}
&((\forall z, (\exists u, p(y, u) \land \neg p(z, u)) \lor (\forall v, \neg p(x, v) \lor p(z, v))) \land \\
&\neg \Delta[P](x, y)
\end{align*}
The only bad thing is this $\forall z$, encode $\forall z$ need encode $\forall p(z,\_)$ and make the query not in EPR. Thus I just want to eliminate this $\forall z$.

As I said, the verity of datatype variable assignment is encoded as the verity of interpretation of predicates, $\forall z$, is actually equal to different value of $\forall p(z,_)$. The domain of predicates is infinite, but the applications of predicates are finite. Then try to enumerate all possible cases:
\begin{enumerate}
    \item Notice the term $\neg p(z, u)$ in formula, try to find the counter formula. If $z \models (\forall u, p(z,u))$ then the body of $\forall z$ above will be
    \begin{align*}
        (\forall u, p(z,u)) \implies (\exists u, p(y, u) \land \neg p(z, u)) \lor (\forall v, \neg p(x, v) \lor p(z, v))
    \end{align*}
    which is
    \begin{align*}
        (\forall u, p(z,u)) \implies (\forall v, \neg p(x, v) \lor p(z, v))
    \end{align*}
    which is equal to $(\forall u, p(z,u)) \implies true$.
    \item $z \models \neg (\forall u, p(z,u))$ which is $z \models \exists u_0, \neg p(z,u_0)$. the body is
    \begin{align*}
        (\exists u_0, \neg p(z,u_0)) \implies (\exists u, p(y, u) \land \neg p(z, u)) \lor (\forall v, \neg p(x, v) \lor p(z, v))
    \end{align*}
    
    Notice the term $p(z, v)$ in formula, try to find the counter formula. If $z \models \exists u, p(z,v)$ then the body of $\forall z$ above will be

    which is
    \begin{align*}
        (\exists v, p(z,v)) \land (\forall u, (\neg p(y, u) \lor p(z, u))) 
    \end{align*}
\end{enumerate}

For a VC: P(x, y) /\ forall u, q(y, z, u) ==> forall v, post(x, z, v)  where  q  and post  are quantifier-free formula over its args. Then, the maximal query is, not (forall z pred(z), (forall u, q(y, z, u)) ==> (forall v, post(x, z, v))) 

==> discuss/result.tex <==
\section{Result}

==> sections/artifact_comments.tex <==
\textbf{Reviewer A:}

\emph{a more permanent deposit of image instead of Docker Hub (e.g., Zenodo) would be useful.}

Per this suggestion, we have uploaded a docker image to Zenodo as well, the URL is Zenodo:10.5281/zenodo.5130646. This image `elrond-2021-oopsla-image.tar.gz` can be loaded by the command:

```
# docker load < elrond-2020-oopsla-image.tar.gz
```

This docker image is the same as the original submitted image:

Dockerhub(elrondinfer/elrond:2021-oopsla): 03faf371d459b81c404b499ef89bff6164409536011776c1f34eabf49a48ed66

Once artifact evaluation is completed, we commit to uploading an image of the artifact after incorporating any feedback from the AEC.

\emph{a method for placing tool outputs in a separate Docker volume (to preserve them even after the container is deleted) would be appreciated.}

Thanks for this suggestion! Indeed, changing the `outputprefix` field in config file works here. To summarize the full instructions for saving outputs outside the container:

1. Run docker with the following command (note there there is a prefix underscore before `\$IMAGE_PATH`)

```
# docker run -v \$HOST_PATH:/home/opam/ADT-Lemma-Discovery/_\$IMAGE_PATH -it elrondinfer/elrond:2021-oopsla
```

2. Set `outputprefix` field in config file to `\$IMAGE_PATH`, replacing `\$IMAGE_PATH` with the location to save the output to.

For example, the following command mounts `/tmp` to `~/_output`:

```
# docker run -v /tmp:/home/opam/ADT-Lemma-Discovery/_output -it elrondinfer/elrond:2021-oopsla
```
And we would then set the `outputprefix` field in `config/standard.config` to:

```json
"outputprefix": "output/benchmark_"
```

Running the benchmarks with our script now saves the results to `/tmp`:

```
# ./bin/run_benchmarks_short.sh
```

We can add a new section with these instructions in the next version of the artifact.

\textbf{Reviewer B:}

\emph{However additional instructions on how to compare the results to the ones presented in the paper would be nice.}

The main results supported by our artifact are the experiments described in Table 4 and Figure 5. The scripts to run benchmarks and replicate the table/figure generation are described in "Running Benchmarks" section of our document. After running these scripts, users should see the same numbers as in the table and similar figures, although total run times may take longer since the tool is running in docker.

\textbf{Reviewer C:}

\emph{Unfortunately, the build of a local image with Dockerfile failed at the following step:}

We encountered a similar z3 installation error when building the docker image with less than 8GB RAM available. The memory error can be fixed by increasing the memory limit in Docker; you can find instructions for doing so on Mac here: (https://docs.docker.com/docker-for-mac/#resources), and for Windows here: (https://docs.docker.com/docker-for-mac/#resources).

\emph{In addition, the source code was provided in the Docker image but there is no compilation instruction.}

The compilation instructions are embedded in our Dockerfile; we will certainly include these in the next version of our instructions.

Specifically, the last three instructions in the Dockerfile compile Elrond.

```
RUN bash ./init.sh
RUN dune build
RUN cp \_build/default/main/main.exe main.exe
```

Users can rebuild the repo in our prebuilt image by first cleaning it:

```
# rm main.exe
# dune clean
# ./init_clean.sh
```

And then compiling:

```
# ./init.sh
# dune build
# cp \_build/default/main/main.exe main.exe
```


==> sections/changes.tex <==
\newpage
\section{Summary of Revisions}

The text corresponding to the major changes is colored \NV{magenta} in our revised version. Typo fixes and minor edits are not highlighted.

\subsection{Restructure Section 2 to be more top-down (Reviewer C)}
\begin{enumerate}
    \item Add an overview in the beginning of \autoref{sec:motivation} to introduce our approach, with additional figures detailing
      the specification inference and weakening procedures (\autoref{fig:specinfer} and \autoref{fig:weakening} resp.).
    \item Include a new detailed description of the main challenges in Section 2.1.
    \item Reiterate and illustrate how we use the approaches introduced in the overview to overcome these challenges.
    \item Simplify \autoref{fig:safe_consistent_maximal} to help introduce the concept of safe/consistent/maximal verification interfaces.
    \item Add more examples (e.g. \autoref{tab:neg2} and \autoref{tab:weaken}, an implementation example illustrating potential definitions of method predicates) to clarify our presentation.
\end{enumerate}

\subsection{Refine the presentation of the algorithm in Section 5 (Reviewer A, C)}
\begin{enumerate}
    \item Add an explicit loop that checks for convergence of weakening in \autoref{algo:multi}.
    \item Change $\I{DiscoverMapping}$ from the original Algorithm 2 to the new specification inference algorithm, in order to fit the changes in \autoref{sec:motivation}.
    \item Add an intuitive explanation of the query from line 3 of \autoref{algo:single}.
    \item Update the explanations of all three algorithms to align with \autoref{fig:specinfer} and \autoref{fig:weakening}.
    \item Simplify terminology and clarify presentation throughout the section.
\end{enumerate}

\subsection{Other changes}
\begin{enumerate}
    \item Clarify the guarantees provided by our system in \autoref{sec:intro}. (Reviewer-C)
    \item Clarify our definition of "maximality", so that maximal verification interfaces are safe and consistent by definition.
          Previously we used "safe, consistent and maximal" to refer to such interfaces. (Reviewer-B)
    \item Clarify the situation with multiple verification conditions in \autoref{sec:formalization}. (All)
    \item Add more examples (e.g. examples illustrating the use of  $\Gamma_F$ and $\Gamma_P$),
          refine old examples (e.g. example of unitary classifiers) and add additional references back to the examples in \autoref{sec:motivation} to explain our
          definitions and theorems in \autoref{sec:formalization} and \autoref{sec:learning}. (All)
    \item Explain the theoretical limitations of our hypothesis space in a footnote in \autoref{sec:learning}. (Reviewer B)
    \item Formalized the definition of the result of weakening algorithm, which we originally referred to as a "maximal specification".  (Reviewer A, C)
    \item Update the theorems and corresponding proofs (\releasesource{}) to align with the revised presentation.
    \item Add comparisons to the suggested related works in \autoref{sec:related}. (Reviewer B)
    \item Fix typos and other minor errors.
\end{enumerate}

% Clarify our guarantees(as our rebuttal).

% Emphasize the novelty(as the overview of our rebuttal).

% \subsection{Changes in Sec 2}

% Restructure Section 2.
% \begin{enumerate}
%     \item start with an overview of the key phases of your approach to describe the big picture, add a new figure here which describes an abstract of our algorithm 1-3, which includes a CEGIS loop.
%     \item give an explicit overview of the key challenges and how you address them.
%     \item then use the example to reiterate and illustrate these points concretely(the old version of Sec 2.)
% \end{enumerate}

% Refine the representation and explanation of the Cex(on line 288), Cex'(on line 415).

% Add a short discussion (~1-2 paragraphs) to the end of Section 2 recapping the pieces the user needed to provide and their roles, including method predicates, and how piece of the example corresponds to a step in the algorithm (i.e. the new figure 2).

% Add a subsection talk about the predicates(as our rebuttal).

% Typos:
% \begin{enumerate}
%     \item "classier" to "classifier" on line 333.
%     \item the ambiguous representation on line 449-452.
%     \item "make" to "makes" on line 468.
%     \item "entails" to "is entailed" on line 470.
% \end{enumerate}

% \subsection{Changes in Sec 3}

% Clarify that we only talk about one VC situation, algorithm for multiple VCs is a straightforward generalization.(as our rebuttal)

% \subsection{Changes in Sec 4}

% Add a short discussion about "Prenex Universally-Quantified Formula"(as our rebuttal).

% Refine the representation of the samples(on line 658).

% Refine the example on line 683-684.

% Clarify the Theorem 4.9(as our rebuttal).

% Typos:
% \begin{enumerate}
%     \item add a "resp." on line 702.
% \end{enumerate}

% \subsection{Changes in Sec 5}

% Add more Input output examples and point back to the overview in Section 2.

% Add a short discussion about our "quantifier increasing" method and grammar based searching(as our rebuttal).

% Refine the representation of weakening until convergence on line 4 in Algorithm 1. Fix the return value of Algorithm 3 when the specification is already maximal on line 861.

% Add an intuitive explanation of the query on line 3 in Algorithm 3(as our rebuttal).

% Add example in weakening inference (Sec 5.3).

% Clarify that the weakening does not involve random generated data(as our rebuttal).

% Typos:
% \begin{enumerate}
%     \item Add the missing first argument on line 8 in Algorithm 3.
%     \item Fix the name "WeakeningLoop" to "Weakening Algorithm"(we have a procedure called "WeakeningLoop" in the old version of the algorithm 3).
% \end{enumerate}

% \subsection{Changes in Sec 6}

% Typos:
% \begin{enumerate}
%     \item \ZZ{The reviewer B is confusing about "Our benchmarks cover a range of abstract data types manipulating a diverse set of algebraic data types", the abstract data types are implemented by the underline algebraic data types, shall we explain a little more here or just say "a range of abstract data types" and omits algebraic data types.}
% \end{enumerate}

% \subsection{Changes in Sec 7}

% Add comparisons to the suggested related works(as our rebuttal).

% Typos:
% \begin{enumerate}
%     \item remove duplicate "provide" on line 1101.
%     \item \ZZ{We say "abducibles" on line 1118 but does not provide the definition(which is a term in abduction, e.g. in MSS paper). We should use another term or add its definition.}
% \end{enumerate}

% \subsection{Changes in Sec 8}

% Typos:
% \begin{enumerate}
%     \item Fix the wrong "lemma" on 1119, 1122 and 1100 to "specification"(The "lemma" is from our old version of paper.)
% \end{enumerate}
% \newpage


==> sections/implementation.tex <==
\section{Implementation}
\label{sec:implementation}

%% \begin{figure}[t]
%% \includegraphics[width=\columnwidth]{figure/workflow_simpfied.png}
%% \centering
%% \caption{\small Overview of \name's workflow.}
%% \label{fig:workflow}
%% \end{figure}

We have implemented a verification pipeline, called \name{}, for the
modular verification of OCaml programs which are clients of libraries
of functions manipulating algebraic data types, shown in
\autoref{fig:workflow_simplified}. Verification conditions for client programs
are generated by weakest liberal precondition predicate
transformers. \name{} does not infer automatically inductive loop
invariants for recursive functions in client programs, and expects
client programs to provide, in addition to any relevant pre- and
post-conditions, any necessary loop invariants. Our implementation is written in $7267$ lines of Ocaml code.

\SJ{LOC of implementation.}

% We derive specifications for library methods used by the client using
% DOrder, a specification inference framework tailored for functional
% data structures~\cite{zhu2016automatically}.
% We infer the specifications $\Delta$ for library function calls which is sufficient to verify a client-supplied post-condition given library specifications along with any pre-conditions, and VCs using an SMT solver. If
% verification fails, \name{} attempts to learn a lemma using
% Algorithm~\ref{fig:algo}. If verification succeeds, the candidate
% lemma can be verified against an implementation of its method
% predicates. \name{} uses the Z3 SMT solver \cite{de2008z3} for its
% satisfiability checking component, $\mathit{IsSat}$.  It implements
% $\I{Learner}$ using the C4.5 decision tree
% algorithm~\cite{ruggieri2002efficient}, and $\I{Sampler}$ using the
% QuickCheck property-based testing
% framework~\cite{claessen2011quickcheck}.

%\subsection{Predicates}

We assume specifications are given using a fixed set of predicates for
the various datatypes supported.  For example, our specification
inference algorithm for libraries whose methods manipulate lists are
expressed in terms of the following predicates:
(a) $\I{hd}(l, u)$: element $u$ is the head of the list $l$; (b)
$\I{mem}(l, u)$: element $u$ is a member of the list $l$; and, (c)
$\I{ord}(l, u, v)$: element $v$ appears after element $u$ in the list $l$, separated by an arbitrary number
      of elements less than or equal to  $\S{length}(l) - 2$.

Our implementation supports inference over stacks, binary
trees, heaps, queues, splay trees, leftist trees, tries, streams and
sets, and provides different predicate sets tailored for that type
used in the specification of libraries.

%% \subsection{A Decision Tree Classifier}

%% A decision tree is a classifier that fully separates positive and
%% negative samples. Decision tree learning uses "information gain" as a
%% measure to learn simpler and more general classifiers that guide our
%% algorithm to infer weaker (aka more general) specifications given a
%% set of positive and negative samples.

%% A decision tree (DT) in specification inference is a binary tree that
%% represents a Boolean combination of a \emph{feature set}
%% $Fset$. Each inner node of the tree is labeled a feature
%% $\tau \in Fset$; this use of DTs is similar to their use in other
%% learning-based program verification and specification inference
%% tasks~\cite{GNP+16,ZMJ18}.  Each leaf of the tree is labeled either
%% positive $+$ or negative $-$.  To evaluate an input feature vector $v$
%% which is an assignment of $Fset$, we trace a path down from the
%% root node of the tree, going to a true branch or a false branch at
%% each inner node whose labeled feature is $\tau$ depending on $v(\tau)$ which
%% is the value of its feature under assignment $v$. The output of the
%% tree on $v$ is the label of the leaf reached by this process.

%% For a given library function $f$, there is an one-to-one mapping between the DT, which is a Boolean
%% combination of features in $Fset(P, f, \vec{u})$, and the
%% hypothesis space $Hyp(P, f, \vec{u})$ realized by adding or
%% dropping universal quantified variables $\vec{u}$ from the prenex.

%% \begin{table}[]
%%  \begin{tabular}{c|cccc}
%% \toprule
%% positive & \multicolumn{1}{l|}{ord(l, u, v)} & \multicolumn{1}{l|}{ord(l,v,u)} & \multicolumn{1}{l|}{mem(l, u)} & mem(l, v) \\
%% \midrule
%% p1       & \multicolumn{1}{l|}{false}          & \multicolumn{1}{l|}{false}        & \multicolumn{1}{l|}{false}        & false        \\
%% p2       & \multicolumn{1}{l|}{true}           & \multicolumn{1}{l|}{true}         & \multicolumn{1}{l|}{true}         & true         \\
%% p3       & \multicolumn{1}{l|}{true}           & \multicolumn{1}{l|}{false}        & \multicolumn{1}{l|}{true}         & true         \\
%% p4       & \multicolumn{1}{l|}{false}          & \multicolumn{1}{l|}{false}        & \multicolumn{1}{l|}{true}         & true        \\
%% p5       & \multicolumn{1}{l|}{false}          & \multicolumn{1}{l|}{false}        & \multicolumn{1}{l|}{true}         & false        \\
%% \midrule
%% negative &                                     &                                   &                                   &              \\
%% \midrule
%% n1       & \multicolumn{1}{l|}{true}           & \multicolumn{1}{l|}{false}        & \multicolumn{1}{l|}{true}         & false        \\
%% n2       & \multicolumn{1}{l|}{true}           & \multicolumn{1}{l|}{false}        & \multicolumn{1}{l|}{false}        & false        \\
%% n3       & \multicolumn{1}{l|}{true}           & \multicolumn{1}{l|}{true}         & \multicolumn{1}{l|}{false}        & false        \\
%% n4       & \multicolumn{1}{l|}{true}           & \multicolumn{1}{l|}{true}         & \multicolumn{1}{l|}{true}         & false        \\
%% \bottomrule
%% \end{tabular}
%% \caption{\small Decision-tree learning samples.}
%% \label{tab:dt}
%% \end{table}


%% \begin{figure}[t]
%% \includegraphics[width=250pt]{figure/dt2.png}
%% \centering
%% \caption{\small Two DTs for the same feature vector set.}
%% \label{fig:dt2}
%% \end{figure}

%% For example, consider the positive and negative feature vectors over the feature set
%% \[\{\I{ord}(l, u, v), \I{ord}(l, v, u),\I{mem}(l, u), \I{mem}(l, v)\}\] shown in \autoref{tab:dt}. One DT is shown in the left-hand side of
%% \autoref{fig:dt2}.  Here, we first pick the feature $\I{mem}(l, u)$
%% as a root to separate the samples $\{p_2,p_3,p_4,p_5,n_1,n_4\}$ and
%% $\{p_1,n_2,n_3\}$.  Neither of these sets are purely positive or
%% purely negative, which means they still need to be refined.  This DT
%% uses four inner nodes and can be mapped to a formula in our hypothesis
%% space by adding the quantified variables $u, v$ to the prenex:
%% \begingroup
%% \setlength{\jot}{0pt}
%% \begin{align*}
%%     \forall u\ v, &(\I{mem}(l, u) \implies (\\
%%     &\quad (\I{ord}(l, u, v) \implies \I{mem}(l, v)) \land\\
%%     &\quad (\neg \I{ord}(l, u, v) \implies \top))) \land \\
%%     &(\neg \I{mem}(l, u) \implies \neg \I{ord}(l, u, v))
%% \end{align*}
%% \endgroup

%% A simpler DT is shown in the right
%% hand side of \autoref{fig:dt2}; this DT uses fewer inner nodes and thus
%% yields a correspondingly shorter formula:
%% \begingroup
%% \setlength{\jot}{0pt}
%% \begin{align*}
%%     \forall u\ v, &(\I{mem}(l, v) \implies \top) \land \\
%%     &(\neg \I{mem}(l, v) \implies \I{ord}(l, u, v))
%% \end{align*}
%% \endgroup
%% This specification has the same meaning as the one shown in the left-hand side
%% in \autoref{fig:dt2}.  However, it uses different \emph{features} for
%% its nodes.

%% Thus, central to our learning task is the question of quantifying a
%% notion of the \emph{goodness} of feature.  Informally, the
%% information gain of a feature evaluates to how homogeneous the
%% feature vectors are after choosing the feature as a separator.  We prefer
%% high information gain features that lead to a split that causes two
%% partitions, one with more positive feature vectors and the other with more negative.  However, there are no guarantees on learning a high
%% information gain split at every internal classification task.

%% The Shannon Entropy $\epsilon$ of a set of feature vectors $\I{FVec} =
%% \I{FVec}^+ \cup \I{FVec}^-$ is:
%% \[\epsilon(\I{FVec}) = -\frac{|\I{FVec}^+|}{|\I{FVec}|}\log_2 \frac{|\I{FVec}^+|}{|\I{FVec}|} - \frac{|\I{FVec}^-|}{|\I{FVec}|}\log_2 \frac{|\I{FVec}^-|}{|\I{FVec}|}\]
%% which yields a value that rates the ratio of positive and negative
%% feature vectors.  A small entropy value indicates that $\I{FVec}$ contains
%% significantly more of one than the other.  Formally, the
%% \emph{information gain} $\I{IG}$ of a feature $\tau \in FSet$ on $\I{FVec}$ is:
%% \begin{align*}
%%     &\I{IG}(\I{FVec}, \tau) = \\
%% &\epsilon(\I{FVec}) - \big( \frac{|\I{FVec}_{\tau}| \epsilon(\I{FVec}_{\tau})}{|\I{FVec}|} + \frac{|\I{FVec}_{\neg \tau}| \epsilon(\I{FVec}_{\neg \tau})}{|\I{FVec}|}\big)
%% \end{align*}
%% where $\I{FVec}_{\tau}$ and $\I{FVec}_{\neg \tau}$ are feature vectors in
%% $\I{FVec}$ that assign $\tau$ to $\C{true}$ and $\C{false}$.

%% For example, the feature $\I{mem}(l, v)$ splits the samples in \autoref{tab:dt}
%% to $\{p_2,p_3,p_4\}$ and $\{p_1,p_5,n_1,n_2,n_3,n_4\}$. This partition
%% is preferable to $\I{mem}(l, u)$, which splits its samples into
%% $\{p_2,p_3,p_4,p_5,n_1,n_4\}$ and $\{p_1,n_2,n_3\}$, because
%% $\I{mem}(l, v)$ separates more positive samples from negative
%% ones. The decision tree algorithm will choose $\I{mem}(l, v)$ as a
%% root and will generate the DT on the right-hand side of
%% \autoref{fig:dt2} because $\I{mem}(l, v)$ has higher information
%% gain.

%% Consider the
%% four features which is represented as separation lines in
%% \autoref{fig:dtsamples},  The decision tree algorithm can use \emph{information gain}
%% as measurement to evaluate the goodness of the feature based on
%% samples, and choose the best feature to generate simpler classifier.


==> sections/rebuttal.tex <==
We thank the reviewers for their detailed comments, and we look
forward to incorporating their feedback in the revised version of the
paper.

Overview:
---------

We emphasize that the primary novelty of our approach is the use of
data to infer plausible explanations (i.e. specifications) of the
behaviors of black-box library functions that ensure the safety of a
client program.  In this sense, we are tackling the same high-level
multi-abduction problem as Albarghouthi et al.  Unlike their work,
however, our setting considers specifications involving algebraic data
types, and must thus work in a different theory (EUF) that unlike
theirs (linear integer arithmetic, (LIA)), lacks a complete abduction
procedure.

Our approach, therefore, uses data in two ways in order to compensate
for the lack of such a procedure: 1) we use concrete runs of black-box
implementations to generate reasonable explanations (i.e. explanations
that are consistent with implementation behavior); and, 2) we limit
overfitting to these samples by using symbolic data from the SMT
solver to ensure they are sufficiently general (i.e. maximally weak).
The use of SMT-generated data for weakening specifications is in sharp
contrast to other data-driven approaches that typically employ
heuristics or rely on a learning procedure (e.g., decision trees) to
drive generalization, and are thus not concerned with finding weakest
specifications.

Our approach guarantees that even in the absence of library source
code, inferred specifications are: 1) *safe* in terms of client
assertions - executing a client using a library implementation that
satisfies these specifications is always safe, and 2) *consistent*
with any observations of library behavior produced from concrete
tests.


Proposed Changes:
-----------------

We propose to make the following modifications to the revision to
address the reviewer's concerns:

- To clarify our presentation, we will add more examples (especially
  for weakening), making space by moving some definitions and theorems
  to a technical report.
- We will refine the presentation of the algorithm in Section 5 to provide
  better intuitions about its design.
- We will add comparisons to the suggested related works (Reviewer-B and -C)
  per the discussion below.

Detailed Response:
-----------------

\textbf{Reviewer A:}

\emph{Dependence on random test generator, and sensitivity/robustness of the technique.}

We concur that, like all data-driven approaches, our algorithm is
dependent on the quality of the underlying data (i.e. the tests
generated by QuickCheck in the case of our initial solutions). It is
precisely for this reason that our algorithm uses a second weakening
phase to ensure that the final abduced specifications are not
overfitted to or otherwise biased by the test generator. Our
evaluation demonstrates how (lines 1067-1069) weakening can
meaningfully combat such biases.

In addition, we observed that the sorts of shape properties (e.g.,
membership, ordering) used by our specifications and assertions are
relatively under-constrained and are thus amenable to property-based
random sampling. We do not ask, for example, for QuickCheck to
generate inputs satisfying non-structural properties like "the $116^{th}$
element of a list is equal to 5''.

\emph{Weakening procedure in Algorithm 1:}

In order to make Algorithm 1 concise, we adopted the convention that
the "forall" on line 4 continues until $\Delta$ converges.  To clarify
this, we will add an explicit loop that performs this convergence
check in the revised version of the paper.

\emph{Theorem 5.2:}

At a high level, \emph{DiscoverMapping} always halts because it
considers a finite space of possible specifications, i.e.  those drawn
from Definition 4.4. At each iteration of the loop, the loop either
terminates or strengthens one of the inferred specifications. Since
there are only a finite number of such specifications, the loop must
eventually terminate. Note that Algorithm 2 is not guaranteed to
terminate, as it can always increase the number of quantified
variables used by the hypothesis space.  The full proof of Theorem 5.2
can be found in the supplemental material (lines 1336 - 1344).  Even
though we do not limit the number quantified variables in our
implementation, our experimental results (the |$\vec{u}$| column in Table
4) show that typically 3 quantified variables are enough to solve our
benchmarks.

\emph{Line 3 of Weakening algorithm (Algorithm 3):}

Intuitively, this query can be interpreted as "there exists a safe
execution (i.e. one that satisfies $\Phi$) consistent with the
candidate specifications besides $\Delta(R_f)$ (the first part of
implication), that is not currently allowed by the specification of $f$
(the second part of implication)". If this statement holds (i.e. the
negation of this implication is UNSAT), then by Definition 3.5, the
weakened specification is maximal. If it does not hold, the
corresponding model represents a safe execution that should be allowed
by the specification of $f$. Such models are examples of the weakening
samples described in Section 4.2.

\textbf{Reviewer B:}

\emph{Related Work:}

Thank you for providing these references.  We will be sure to provide a
detailed comparison in the revised version.  To clarify the differences
between our work and these:

- Like our setup, J. Su et al's work extended from H.A. Nguyen et
  al. infers specifications of library APIs from client information.
  However, they try to infer correct library specifications under the
  assumption that client is correct. On the other hand, we do
  abduction to provide guarantees that any library implementation must
  satisfy to ensure the client is safe.  Our approach does not assume
  clients are always safe - e.g, Elrond was able to identify safety
  violations in 5 of our benchmarks(lines 1007-1010).  Another distinguishing feature
  in our work is the focus on generating maximally weak specifications to
  overcome generating overfitted specifications.

- S. Qin et al. also infer specifications for unknown procedures in a
  rich domain involves the shape property of datatypes. However,
  because their technique does not involve any queries to the library
  implementation and does not do weakening like ours, inferred
  specifications may be over-fitted to the client safety property;
  e.g., their approach may fail to infer a specification that admits
  duplicate stack elements (lines 432-435).  In contrast to our work, their
  method also requires users to understand the underlying
  representation of the datatype used by the library method, and
  present explicit interpretations of predicates used in
  specifications sufficient to verify the client.  Finally, unlike
  Qin, we provide an algorithmic weakening procedure to refine
  inferred specifications.

- The work of R. Pandita et al. learns specifications from comments in
  natural language but does not provide safety and consistency
  guarantees, as discussed in the overview section above.

\emph{(1) Method Predicates:}

Method predicates are provided by the user.  In our example, we might
implement predicates \emph{hd} and \emph{mem} as:


   fun \emph{hd}($\textsf{s, u}$) = ($\textsf{Stack.top s = u}$)

   fun \emph{mem}($\textsf{s, u}$) = ($\textsf{Stack.top s = v}$) || \emph{mem}($\textsf{Stack.pop s, v}$)


While it is possible to naively translate each library method as a
predicate, such an approach may not be useful for verification.  Some
functions may be irrelevant to client assertions, unnecessarily
increasing the hypothesis space from which specifications are drawn.
Conversely, the library may not include functions for desirable
predicates; e.g., the Stack library does not provide a $\textsf{Stack.mem}$
function that is nonetheless relevant for verifying our running
example.  Notably, we impose no restriction on the structure of method
predicates - observe that the definition of \emph{mem} is recursive, and that
both $\mathsf{Stack.top}$ and $\mathsf{Stack.pop}$ refer to black-box implementations of Stack library
methods.

\emph{(2) Prenex Universally-Quantified Formula:}

As with any automated verification exercise, we face a tradeoff
between expressive power and algorithm efficiency; we chose to
constrain our specifications in this way in order to ensure that our
SMT queries were in the decidable EPR fragment. As verification
technology improves, we could certainly relax this
restriction. EPR-based encodings are commonly used in practice, and
was expressive enough for all our benchmarks.

The main sorts of properties that we do not support as a consequence of this choice
are those which use quantifier alternation, e.g. "for every element in
a stream, there exists another larger element that appears after than
it" ($\forall u, \exists v, \mathit{mem}(l,u) \implies (\mathit{mem}(l,v) \land
\mathit{ord}(l,u,v) \land u \le v)$).

\textbf{Reviewer C:}

\emph{(1) Understanding the counter-example (CEX) and method predicates}

CEX is a model produced by the Z3, and it provides interpretations to
the query's uninterpreted predicates (in this case \emph{hd}
and \emph{mem}) as anonymous functions (see below).  Even though we have
implementations of these predicates, directly encoding their semantics
in logic is problematic given e.g., the recursive structure of
\emph{mem}.  Thus, the theorem prover views these predicates as
uninterpreted and therefore the models it generates
may well be inconsistent with their actual semantics.


As an example, one possible SMT model for the CEX given on line 288
is:

$\nu_{top}$ = $19$

$\nu$ = $1$

$\nu_{concat}$ = $2$

$\nu_{tail}$ = $3$

\emph{hd} = $\lambda l, u. false$

\emph{mem} = $\lambda l, u. \text{if }(l = 1 \lor l = 2 \lor l = 3) \land u = 19 \text{ then } true \text{ else } false$

Algebraic datatypes are encoded as integers, and we replace the $1$,
$2$, and $3$ in the interpretation of \emph{mem} with $\nu$,
$\nu_{concat}$ and $\nu_{tail}$ when presenting CEX in the paper.

\emph{(2) Role of quantified variables:}

Many of our method predicates are relational; increasing the number of
quantified variables broadens our hypothesis space to include richer
relationships: expressing transitivity, for example, require at least
three quantified variables: $\forall u,v,w. \mathit{ord}(l,u,v) \land
\mathit{ord}(l,v,w) \implies \mathit{ord}(l,u,w)$. Similarly, any binary predicate,
e.g. \emph{mem}$(l,u)$, requires 2 quantified variables.  Using a
grammar of predicates with increasing size bounds to encode the
hypothesis space is equivalent to our approach, we choose increasing
quantified variables to more closely align with our definition of
maximality (Definitions 3.5 and 3.6).

\emph{(3) Concrete tests in weakening:}

The weakening phase does not check if there is a concrete test
corresponding to the logical samples produced by the SMT solver; since
weakened specifications are guaranteed to preserve safety, this will
not compromise the soundness of our algorithm. Where there is no
corresponding test, we will have weakened the specification to cover a
vacuously true scenario. 

\emph{Comparison to prior work on data-driven invariant inference:}

Broadly speaking, our approach differs from prior work on data-driven
invariant inference insofar as we cannot appeal to any source of
ground truth (e.g, SMT verification (e.g,. Padhi et al., PLDI'16), or
bounded model checking (Miltner et al., PLDI'20)).  This leads to the
need for a weakening procedure to facilitate generalization to
ultimately aid client-side verification.  We believe that techniques
like Miltner et al. can be complementary to ours, using our abduced
specifications to infer and verify representation invariants.

\emph{Compared to CHC solving:}

While it is possible to frame our problem as an instance of CHC
solving (e.g., Zhu et al. (PLDI'18)), we would still be left with the
important challenge of generating maximally weak specifications.  As
observed by Albarghouthi et. al, "...Horn clauses does not address the
question of optimality and would allow trivial solutions that set
unconstrained predicates to false, as allowed by Horn-clause
semantics. In contrast, our multi-abduction solver ensures that we
compute maximal, non-trivial solutions..." (p. 800)

\emph{VC generation:}

We infer VCs for each control flow path, and our full algorithm considers
the conjunction of all these VCs at once. To keep the description of
the algorithms in Sections 3-5 concise, we only consider a single VC
on Sec 3-5; the complete algorithm for multiple VCs is a
straightforward generalization of this approach and is provided in the
supplemental material. This is currently noted in the footnote on page
16, but we will clarify this point in the revised version.

\emph{Negative/positive samples:}

The statement of Theorem 4.9 quantifies over the \emph{entire} space
of negative samples, and every positive sample generated by random
testing (this is what the phrase "entailed by $\Gamma_F$ and
$\Gamma_P$" means). The former ensures that our specifications rule
out every unsafe execution, while the latter ensures they are
consistent with our observations of the libraries' behavior.

\emph{Comparison to Bastani et. al (POPL'15)}

While their work considers a similar problem to ours, analysis of
clients when some pieces of code are missing, discovering minimal
sufficient assumptions, there are several major differences between
our approaches: 1) their specification domain is limited to CFL
reachability (alias and taint specifications), while our hypothesis
space involves shape properties (membership, ordering...)  over
algebraic datatypes; 2) we guarantee specification consistency with
respect to our observations on the black-box implementation of the
libraries; and, (3) they do not provide an explicit weakening
procedure to generalize their solution.

==> sections/review-reference.tex <==
Specification Inference Using Context-Free Language Reachability(Osbert Bastani. POPL 15')

This paper has the similar problem set up with us: do verification and analysis on client side when some pieces of code is missing. However there are still several differences.
Specification domain is limited in CFL reachability(alias specification and taint specification). Our specification space involves shape property rich over datatype.
The inferred specification set is a minimal set of sufficient assumptions for the all potential taints, but is not consistent with the actual implementation of the libraries. Our inferred specifications are consistent with our observation, thus make inferred specifications more close to user's expectation.
The inferred specification needs the human to refine or confirm its correctness(even these specification is not totally correct). \ZZ{Not sure: Our experiment shows our tool is automated and the inferred specifications can be verified against the implementation of libraries.}

"Poster: Using Consensus to Automatically Infer Post-conditions" by J. Su, M. Arafat and R. Dyer (ICSE 2018) and "Mining Preconditions of APIs in Large-Scale Code Corpus" by H.A. Nguyen, R. Dyer, T.N. Nguyen and H. Rajan (FSE 2014)

These works and us both infer specifications of library APIs from the client information, however the goal and assumption of us are different: they try to infer correct specifications of library with the assumption that the usage of client side is correct, on the other hand, we do abduction which guarantees any library implementation satisfies our abduced specifications are safe with respect to the client verification and we have no assumption of the correctness of client code. The quality of the inferred specification is also the common problem we are facing: their work may infer irrelevant or too strong specifications, however, we use the samples to guarantee the consistency of our observation and use weakening procedure to weaken the too strong specifications.
